Self-Improving Autonomous Underwater Manipulation

Underwater robotic manipulation faces significant challenges due to complex fluid dynamics and unstructured environments, causing most manipulation systems to rely heavily on human teleoperation. In this paper, we introduce AquaBot, a fully autonomous manipulation system that combines behavior cloning from human demonstrations with self-learning optimization to improve beyond human teleoperation performance. With extensive real-world experiments, we demonstrate AquaBot's versatility across diverse manipulation tasks, including object grasping, trash sorting, and rescue retrieval. Our real-world experiments show that AquaBot's self-optimized policy outperforms a human operator by 41% in speed. AquaBot represents a promising step towards autonomous and self-improving underwater manipulation systems. We open-source both hardware and software implementation details.

==> old.tex <==

intro version 3

--------------------------

Despite high demand and continuous efforts, a fully autonomous manipulation system is still out of reach for most of critical underwater applications. What makes underwater manipulation so hard? %
In addition to the typical difficulties faced by robotic manipulation systems, underwater robots encounter unique challenges posed by the high-dimensional and nonlinear fluid dynamics. Such complexity in modeling is further exacerbated by the   wide variety of objects, tasks, and environments encountered underwater. This leads to significant challenge in controller design for underwater manipulation.  

As a result, many hand-engineered robotics manipulation systems fall short when attempting to explicitly model the complex dynamics of both the robot and its environment. On the other hand, teleoperated systems \cite{7742315, stuart2017ocean, brantner2021controlling} benefit from human adaptability, allowing them to handle unpredictable conditions and execute complex tasks. 

However, teleoperation is not the perfect solution. First, its scalability is constrained by its dependence on human input. Furthermore, the system's performance is inherently capped by the operator's skill level, which is often suboptimal. For instance, operators frequently opt to substantially reduce vehicle speed when executing precise manipulation tasks, which may not be necessary for an optimal system.  

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/teaser.pdf}
    \caption{AquaBot learns end-to-end visuomotor policies to perform diverse underwater manipulation tasks fully autonomously.}
    \label{fig:teaser}
\end{figure}

This raises a critical question: Can we distill the strategies demonstrated by human operators into a robust and reactive visuomotor policy that enables autonomous execution of manipulation tasks under complex dynamics? Furthermore, can the robot system continuously improve its learned policy through self-guided exploration and optimization, thereby exceeding the performance of human operators?

To answer this question, we propose AquaBot, a system designed to learn end-to-end visuomotor policies for fully autonomous underwater manipulation that can improve beyond human teleoperation performance through self-learning. The training process consists of two stages:
\begin{itemize}
    \item In the first stage, we \textbf{distill human adaptability} into a closed-loop visuomotor policy. To do so, we record human demonstrations that teleoperate the robot to perform various manipulation tasks and then use the data to train a visuomotor policy. By shortening the policy's action horizon, we effectively increase the reactiveness of the policy, which is critical in dealing with unexpected underwater dynamics. 


    \item  In the second stage, we allow the robot to \textbf{self-improve the learned policy} through self-guided optimization. In this step, we repeatedly execute the learned policy and use the execution time as a reward to accelerate the policy with a surrogate-based optimization algorithm. This step allows the system to further optimize those suboptimal parameters (e.g., execution speed) in the human demonstration data. 
\end{itemize}


To evaluate the system, we set up a real-world platform based on commercial and accessible hardware. 
\todo{Talk about the tasks.... On three challenging tasks, such as object grasping, garbage sorting, and large object retrieval. }
Extensive real-world experiments demonstrate that AquaBot can learn a diverse set of manipulation skills from human demonstrations, and self-learning can further improve these learned skills to achieve superhuman performance 
\todo{be more concrete, achieve xx\% better than human teleoperation performance. }



intro version2 

Many tasks involving underwater manipulation, from construction to deep-sea exploration, are conducted by human divers, which presents substantial safety risks due to harsh and unpredictable conditions. These environments are not only dangerous but also limit the duration and scope of tasks that can be completed manually. Autonomous underwater robots offer a promising solution to these challenges. By replacing or assisting human divers, robots can perform complex tasks such as assembling underwater structures, repairing pipelines, or retrieving deep-sea samples, all while minimizing human exposure to hazardous situations.


While exciting progress has been made in robotic manipulation in recent years, underwater manipulation remains a challenging problem. One of the main difficulties is dealing with the dynamic forces of water, such as currents, turbulence, and varying pressure, which can destabilize robots and reduce the precision of their movements. To address these challenges, current autonomous underwater manipulation systems typically rely on modular, hand-engineered components for dynamic modeling, control, motion planning, and perception, each designed to handle specific aspects of the task.

On the other hand, recent advances in the teleoperation of underwater robots have showcased more sophisticated manipulation capabilities. Notably, projects like Ocean One~\cite{} have demonstrated the ability of human operators to achieve complex manipulation tasks, surpassing the skills provided by traditional model-based controllers. This raises a critical question: rather than complicated systems for dynamics modeling, control, and planning, could we instead leverage learning-based methods to learn an end-to-end visuomotor policy from human demonstrations for autonomous underwater manipulation?

However, a key limitation of learning solely from human demonstrations is that the learned policy is inherently constrained by the performance of the human operator, particularly in tasks where speed and precision are critical. To overcome this, it is necessary for the learned policy to further improve from self-exploration, enabling it to exceed the base policy learned from human demonstrations.

--------------------------

We present a system for fully autonomous underwater manipulation using an end-to-end visuomotor policy that can further improve its efficiency through self-learning. Traditionally, underwater manipulation relies on specialized arm-based underwater robots and model-based controllers for positional control of the end-effector, making it expensive to set up and work with. In this work, we adopt a cheap commercial underwater drone with a single protruding gripper and learn an end-to-end visuomotor policy for force/torque control with behavior cloning to achieve autonomous manipulation. With the observation that water provides a safe exploration environment for robots, we propose a self-learning algorithm to accelerate the learned policy. Qualitative and quantitative experiments show that \textit{behavior cloning} can learn end-to-end visuomotor policies to perform a diverse set of underwater manipulation tasks, and \textit{self-learning} can accelerate the learned policies beyond human teleoperation performance.

Learning-based methods such as behavior cloning have emerged to be the dominant method for learning real-world manipulation policy in unstructured environment on-land. Can we apply them to underwater manipulation? Replacing the air in space with water changes fundamental assumptions we usually make for robotic manipulation. These differences can be summarized as follows:
\begin{itemize}
    \item \textbf{Buoyancy} Robots typically float freely in water instead of being mounted on a fixed platform, creating difficulty for precise positional control of the end-effector.
    \item \textbf{Dynamics} The dynamic nature of the water environment causes the outcome of robot actions to be more stochastic, adding challenges to long-horizon planning.
    \item \textbf{Safety} The viscosity and friction from water create a safer environment for self-exploration without extensive safety measures required for on-land operation.
\end{itemize}

\textcolor{red}{Carl: should mention that demonstrations are more challenging to collect up front, this will motivate self-learning}

To cope with these differences, we propose a system and a learning method tailored for underwater manipulation:
\begin{itemize}
    \item \textbf{Force/torque Control} Instead of the default end-effector position control, which is difficult to achieve with high-precision underwater, we use behavior cloning to learn a visuomotor policy for force and torque control.
    \item \textbf{Lightweight Policy} Instead of predicting long-horizon action trajectory, we choose to use a lightweight policy for a higher re-plan frequency and a shorter prediction horizon.
    \item \textbf{Self-learning} We adopt a self-learning framework for learning to improve the learned manipulation policy, which is essential to underwater manipulation where human teleoperation skill is sub-optimal.
\end{itemize}

Hardware-wise, we choose to use an underwater drone with a single protruding gripper for manipulation instead of traditional hardware based on a large underwater vehicle where a robotic arm with multiple joints is mounted. Our hardware choice poses several advantages compared to traditional hardware while being orders of magnitudes cheaper. Instead of operating under the kinematic constraints and operating range of the robot arm, our drone-gripper system can move freely in all directions without any kinematic constraints. Instead of a complicated controller for both the mounting vehicle and the robot arms with high-dimensional control space, our drone-gripper system equates the robot movements with the gripper movements. Instead of many moving parts and complicated protrusions requiring specialized waterproof solutions, our drone-gripper system is a one-piece rigid body with a single protruding gripper, significantly strengthening the structural integrity of the system.

\textcolor{red}{Carl: Not sure I am buying the emphasis on low-cost. Yes, it's good for research and experimentation, but unlike home robotics, a robot in the field needs to be built tough in practical settings anyways to withstand everything. What does cheap underwater robots enable beyond pool cleaning?}

The choice of our hardware platform and design decisions of our learning method massively simplify the traditionally complicated, specialized, and expensive underwater manipulation system. We demonstrate in our experiments that our proposed system can be used to learn a diverse set of manipulation skills, including object grasping, garbage sorting, and people rescuing. We believe our contribution will shift the paradigm for autonomous underwater manipulation, democratizing this traditionally specialized domain, and inspiring on-land manipulation researchers to explore new learning methods for underwater manipulation, 

-------------------------------

